Value-centric Dynamic Partial Order Reduction

The verification of concurrent programs remains an open challenge, as thread interaction has to be accounted for, which leads to state-space explosion. Stateless model checking battles this problem by exploring traces rather than states of the program. As there are exponentially many traces, dynamic partial-order reduction (DPOR) techniques are used to partition the trace space into equivalence classes, and explore a few representatives from each class. The standard equivalence that underlies most DPOR techniques is the happens-before equivalence, however recent works have spawned a vivid interest towards coarser equivalences. The efficiency of such approaches is a product of two parameters: (i) the size of the partitioning induced by the equivalence, and (ii) the time spent by the exploration algorithm in each class of the partitioning. In this work, we present a new equivalence, called value-happens-before and show that it has two appealing features. First, value-happens-before is always at least as coarse as the happens-before equivalence, and can be even exponentially coarser. Second, the value-happens-before partitioning is efficiently explorable when the number of threads is bounded. We present an algorithm called value-centric DPOR (VCDPOR), which explores the underlying partitioning using polynomial time per class. Finally, we perform an experimental evaluation of VCDPOR on various benchmarks, and compare it against other state-of-the-art approaches. Our results show that value-happens-before typically induces a significant reduction in the size of the underlying partitioning, which leads to a considerable reduction in the running time for exploring the whole partitioning.

==> comparison.tex <==
\section{Comparison with other DPOR approaches}\label{sec:comparison}
In this section we illustrate the differences between our algorithm with other recent DPOR approaches.
First, we compare with algorithms present in our experimental evaluation, namely,
$\Source$, $\Optimal$~\cite{Abdulla14}, $\OptimalObs$~\cite{Aronis18}, and $\DCDPOR$~\cite{Chalupa17}.
Then, we further discuss differences with $\MCR$~\cite{HUANG15} and $\CSDPOR$~\cite{Elvira17}.


\subsection{Comparison with $\Source$, $\Optimal$~\cite{Abdulla14},\\and $\OptimalObs$~\cite{Aronis18}}

The work~\cite{Abdulla14} introduces two DPOR approaches, namely, $\Source$ DPOR and $\Optimal$ DPOR,
both of which are based on the Mazurkiewicz trace equivalence $\Maz$.
First, the work introduces the notion of \emph{source sets}, which replace the previously considered persistent sets,
and presents a DPOR algorithm that uses source sets, i.e., $\Source$. Second, the work further introduces the data
structure called \emph{wakeup trees} and proposes an algorithm $\Optimal$ that uses both source sets and
wakeup trees, and is optimal in the sense that it explores exactly one trace per Mazurkiewicz equivalence class.
Finally, the work of~\cite{Aronis18} presents Optimal DPOR with Observers ($\OptimalObs$).
The algorithm is also based on Mazurkiewicz equivalence, but it uses the notion of \emph{observers} to 
avoid exploring certain Mazurkiewicz classes while remaining sound for bug finding.

\smallskip\noindent{\bf Comparison with $\VCDPOR$.}
The trace partitioning $\VHB$ constructed by $\VCDPOR$ is provably coarser than $\Maz$ constructed by $\Source$
and $\Optimal$ (see~\cref{them:comparison}). The partitioning $\VHB$ is incomparable with the partitioning
explored by $\OptimalObs$.
In the example program~\cref{fig:motivating_example} given in the introduction~(\cref{subsec:example}), both $\Source$
and $\Optimal$ explore all four traces, whereas $\OptimalObs$ explores three traces (referring to the example description,
$\OptimalObs$ will not explore either $\Trace_1$ or $\Trace_2$, as the race they differ in is unobserved). In the
example~\cref{subfig:m_comparisona} given in~\cref{sec:ave}, $\Source$ and $\Optimal$ explore exponentially many
traces, as demonstrated in the description. $\OptimalObs$ also explores exponentially many traces (although fewer
than $\Source$/$\Optimal$), since exponentially many orderings of writes in thread~$\Process_{1}$ and reads
in thread~$\Process_{2}$ have to be accounted for. In both examples $\VCDPOR$ explores exactly one trace.

While $\Optimal$ and $\OptimalObs$ are optimal for the Mazurkiewicz partitioning, in the worst case, $\Source$ can explore
the same Mazurkiewicz class exponentially many times. This has been independently reported
in~\cite{AbdullaAJS17} and~\cite{Nguyen18}. On the other hand, both $\Optimal$ and $\OptimalObs$ use the
data structure of wakeup trees, the size of which can grow exponentially and thus the memory complexity becomes
exponential in the worst case (further details are reported in~\cite{AbdullaAJS17}). We have seen this phenomenon
arise during our experiments, where in several benchmarks (with three threads) the memory usage of $\Optimal$
and $\OptimalObs$ was orders-of-magnitude higher than that of $\Source$, revealing the exponential space costs of the wakeup trees.
On the other hand, our algorithm $\VCDPOR$ has a guaranteed polynomial complexity per each maximal class 
of the $\VHB$ partitioning.
Further, $\VCDPOR$ is guaranteed to use polynomial space (c.f.~\cref{rem:recursive}).



\subsection{Comparison with $\DCDPOR$~\cite{Chalupa17}}

The work of~\cite{Chalupa17} introduced the observation equivalence $\Observation$, which states that two traces $\Trace_1,\Trace_2\in \TraceSpace$ are
equivalent, written $\Trace_1\ObsE \Trace_2$, if 
(i)~$\Events{\Trace_1}=\Events{\Trace_2}$ and
(ii)~$\Observation_{\Trace_1}=\Observation_{\Trace_2}$.
In words, the two traces are equivalent if they consist of the same set of events and every read event observes the same write event in both traces.
However, $\DCDPOR$ uses the observation equivalence only for a special case of concurrent programs represented as ``acyclic topologies''.
For arbitrary programs, $\DCDPOR$ uses another equivalence, $\ObservationC$, which refines $\Observation$.
Since $\VCDPOR$ is stated for arbitrary topologies (that may have cycles), here we compare $\VHB$ with $\ObservationC$.
We re-state $\ObservationC$ below, and show that $\VHB$ is at least as coarse as $\ObservationC$, and can be become even exponentially coarser.


\smallskip\noindent{\bf The equivalence $\ObservationC$ for cyclic topologies.}
Two traces $\Trace_1,\Trace_2\in \TraceSpace$ are called \emph{cycle-observation-equivalent}, written $\Trace_1\ObsEC \Trace_2$, if the following  hold.
\begin{compactenum}
\item\label{item:obs_c_e} $\Events{\Trace_1}=\Events{\Trace_2}$.
\item\label{item:obs_c_o} $\Observation_{\Trace_1} = \Observation_{\Trace_2}$.
\item\label{item:obs_c_m} $\HB{}{\Trace_1}{}\Project{\SysLeafEvents} = \HB{}{\Trace_2}{}\Project{\SysLeafEvents}$, i.e., $\HB{}{\Trace_i}{}$ agree on the events of the leaf threads.
\end{compactenum}
We note that the observation equivalence $\Observation$ is identical to $\ObservationC$ without \cref{item:obs_c_m} above.
Hence $\ObservationC$ refines $\Observation$.


\begin{restatable}{theorem}{themcomparisondc}\label{them:comparison_dc}
$\VHB$ is at least as coarse as $\ObservationC$, and there exist programs where $\VHB$ is exponentially coarser.
\end{restatable}
\begin{proof}
We first show that $\VHB$ is at least as coarse as $\ObservationC$.
Consider two traces $\Trace_1, \Trace_2\in \TraceSpace$ such that $\Trace_1\not \VHBE \Trace_2$.
If $\Events{\Trace_1}\neq \Events{\Trace_2}$ or $\HB{}{\Trace_1}{}\Project{\SysLeafEvents} \neq \HB{}{\Trace_2}{}\Project{\SysLeafEvents}$ then $\Trace_1\not \ObsEC\Trace_2$ directly by definition.
Else, if $\Value_{\Trace_1}\neq \Value_{\Trace_2}$ or $\SideAnnotation_{\Trace_1}\neq \SideAnnotation_{\Trace_2}$,  we have $\Observation_{\Trace_1}\neq \Observation_{\Trace_2}$.
Else, if $\CHB{}{\Trace_1}{}\neq \CHB{}{\Trace_2}{}$, there exists a read event such that $\Observation_{\Trace_1}(\Read)\neq \Observation_{\Trace_2}(\Read)$.
Hence, in all cases we obtain $\Trace_1\not \ObsEC \Trace_2$.


We now turn our attention in showing that $\VHB$ can be exponentially coarser than $\ObservationC$.
Indeed, consider the example programs of \cref{fig:m_comparison}, for which we have already argued in \cref{sec:ave}
that $\VHB$ is exponentially coarser than $\Maz$.
It is easy to see that for both examples, $\Maz$ coincides with $\Observation$, and since we have only two threads, $\Observation$ coincides with $\ObservationC$.
Hence, in both examples $\VHB$ is exponentially coarser than $\ObservationC$.
The desired result follows.
\end{proof}




\subsection{Comparison with $\MCR$~\cite{HUANG15}}

The work of~\cite{HUANG15} moves away from the Mazurkiewicz equivalence and considers a coarser trace equivalence that is based on
\emph{maximal causal models}. The algorithm $\MCR$ utilizing this equivalence has been implemented in a stateless model checker for
Java and it has proven to be practically very effective, revealing several new errors in well-studied real-world programs.

The maximal-causality equivalence is coarser than the $\VHB$ equivalence used by our $\VCDPOR$. The algorithm $\MCR$ is able to utilize such a coarse
equivalence by employing satisfiability modulo theories (SMT) solvers to realize given maximal causal models. These solvers are NP-oracles,
although recent research has made them perform impressively well in practice. On the other hand, our $\VCDPOR$ has a polynomial
guarantee on the realizability of annotated partial orders (c.f.~\cref{them:closure}), which can be seen as the counterpart of maximal
causal models.

In $\MCR$, whenever new interleavings are discovered that have to be explored (called \emph{seed interleavings}), the recursion
subtrees corresponding to these explorations no longer share any information between each other. This is practically very useful, as
it makes exploration with different seed interleavings embarrassingly parallel. However, to our understanding, this makes $\MCR$ visit the same
trace-partitioning class exponentially many times in the worst case.
On the other hand, our algorithm $\VCDPOR$ has a guaranteed polynomial complexity per each maximal class 
of the $\VHB$ partitioning.

In a follow-up work~\cite{Huang017}, the algorithm $\MCR$ is improved upon by using static-analysis techniques to construct smaller
SMT queries during the exploration. While this does not release $\MCR$ from the need of using an NP-oracle, it provides further
practical speed-up since smaller queries can typically be solved faster by the SMT solvers.
We find it interesting future work to combine our approach with $\MCR$, so that we use the $\MCR$ partitioning (and the expensive SMT solver) only for classes that are exponentially coarser than the $\VHB$ partitioning, and rely on our $\VCDPOR$ algorithm otherwise.


% The example in DCDPOR
% http://lara.epfl.ch/~pavlogia/publications/papers/popl18a.pdf
% is wrong, $\MCR$ does NOT hit the same class exponentially many times



\subsection{Comparison with $\CSDPOR$~\cite{Elvira17}}

The work~\cite{Elvira17} develops an extension of Source DPOR~\cite{Abdulla14} that utilizes \emph{context-sensitive independence} to achieve
coarser trace-space partitioning. On a technical level, context-sensitivity is attained by checking for a reversible race, whether the program state
after reversing the race equals the program state without the reverse. If this is the case, the sequence corresponding to the race reverse does not have
to be explored and soundness is maintained. Thus the sleep set of the corresponding ancestor in the recursion tree is populated with the sequence.

\smallskip\noindent{\bf Comparison with $\VCDPOR$.}
The $\CSDPOR$ technique is not optimal with respect to the partitioning it explores. In particular, it can explore the same partition class
exponentially many times in the worst case. On the other hand, $\VCDPOR$ has a guaranteed polynomial upper bound on the number of
explorations for every class of the $\VHB$ partitioning (c.f.~\cref{lem:vcdpor_complexity} in~\cref{sec:app_vcdpor_proofs}).

The $\VHB$ partitioning is incomparable with the partitioning proposed by $\CSDPOR$ in terms of coarseness. We note that for the example
program~\cref{fig:motivating_example} given in the introduction~(\cref{subsec:example}), $\CSDPOR$ explores more traces
than $\VCDPOR$. In particular, $\CSDPOR$ has to explore both orderings of commands $\Process_{1} : 1.~\Write(x,1)$ and $\Process_{2} : 1.~\Write(x,2)$
(since the commands are dependent and the program states differ in both orderings), whereas $\VCDPOR$ explores exactly one trace.
%The example can be easily extended so that $\VCDPOR$ explores exponentially fewer traces than $\CSDPOR$.\todo{create ex.}
This behavior can be easily extended as in \cref{subfig:csdpor_exptraces_example} so that $\CSDPOR$ explores exponentially many
traces, as all orderings of writes in thread~$\Process_{1}$ and first $n$ writes in thread~$\Process_{2}$
have to be accounted for. 
In contrast, $\VCDPOR$ explores exactly one maximal trace.


\smallskip\noindent{\bf Exponential space usage.}
Since $\CSDPOR$ stores in the sleep sets sequences of steps instead of single-steps, it suffers from exponential space complexity
in the worst case, and is thus not purely a stateless method. 
To see this, consider the simple program given in~\cref{subfig:csdpor_expmem_example}.
We assume a salient write event at the beginning of the program that assigns value $0$ to every variable. 
Now consider an exploration of $\CSDPOR$ such that whenever multiple
threads are enabled at a certain recursive step, the enabled thread with the smallest i.d. performs a step
(i.e., $\Process_{1}$~before~$\Process_{2}$ and $\Process_{2}$~before~$\Process_{3}$). 
The leaves of the recursion tree are traces $\Trace_i=\Read(y)\circ \ov{\Trace}_i \circ \Write(y,0)$,
where $\circ$ denotes concatenation and $\ov{\Trace}_i$ denotes one among the (exponentially many) orderings of the events that write to $x$.
Now consider the root of the recursion tree.
For every such trace $\Trace_i$, $\CSDPOR$ adds the sequence $\ov{\Trace}_i \circ \Write(y,0) \circ \Read(y)$ to the sleep set of the root.
Thus, the sleep set of the root becomes exponentially large, and $\CSDPOR$ uses exponential space.
In contrast, our $\VCDPOR$ uses polynomial space (see \cref{rem:recursive}).


\input{figures/csdpor_expmem_example}

%{\bf Andreas to Viktor: 
%\begin{enumerate}
%\item Fill citation
%\item Remind them that the introductory example shows that $\CSDPOR$ can explore a larger partitioning
%\item Fill example with exponentially large source sets
%\end{enumerate}
%}


==> figures/csdpor_expmem_example.tex <==
\begin{figure}
\small
\begin{subfigure}[b]{0.35\textwidth}
\begin{subfigure}[t]{0.15\textwidth}
\begin{align*}
\text{Th}&\text{read}~\Process_{1}:\\
\hline\\[-1em]
1.~& \Write(x,1)\\
2.~& \Write(x,1)\\
\,& \dots\\
n.~& \Write(x,1)
\end{align*}
\end{subfigure}
\quad
\begin{subfigure}[t]{0.15\textwidth}
\begin{align*}
\text{Thread}&~\Process_{2}:\\
\hline\\[-1em]
1.~& \Write(x,2)\\
%\,& \dots\\
%n.~& \Write(x,2)\\
%n+1.~& \Write(x,1)\\
2.~& \Read(x)\\
\,& \dots\\
n+1.~~& \Read(x)
\end{align*}
\end{subfigure}
\caption{A simple program for which $\CSDPOR$ explores exponentially many traces.}
\label{subfig:csdpor_exptraces_example}
\end{subfigure}
\qquad
\centering
\begin{subfigure}[b]{0.55\textwidth}
\begin{subfigure}[t]{0.15\textwidth}
\begin{align*}
\text{Th}&\text{read}~\Process_{1}:\\
\hline\\[-1em]
1.~& \Read(y)\\
\end{align*}
\end{subfigure}
\qquad
\begin{subfigure}[t]{0.15\textwidth}
\begin{align*}
\text{Th}&\text{read}~\Process_{2}:\\
\hline\\[-1em]\
1.~& \Write(x,n+1)\\
2.~& \Write(x,n+2)\\
\,~& \dots\\
n.~& \Write(x,n+n)\\
\end{align*}
\end{subfigure}
\quad
\begin{subfigure}[t]{0.15\textwidth}
\begin{align*}
\text{Threa}&\text{d}~\Process_{3}:\\
\hline\\[-1em]\
1.~& \Write(x,1)\\
2.~& \Write(x,2)\\
\,~& \dots\\
n.~& \Write(x,n)\\
n+1.~& \Write(y,0)\\
\end{align*}
\end{subfigure}
\caption{A simple program for which $\CSDPOR$ uses exponential space.}
\label{subfig:csdpor_expmem_example}
\end{subfigure}
\caption{Simple examples where $\CSDPOR$ explores exponentially many traces (\protect\cref{subfig:csdpor_exptraces_example}) and uses exponential space (\protect\cref{subfig:csdpor_expmem_example}).}
\label{fig:csdpor_examples.}
\end{figure}


==> figures/fig_comparison2.tex <==
\begin{figure}[]
\small
\centering
\begin{subfigure}[t]{0.15\textwidth}
\begin{align*}
\text{Thread}&~\Process_{1}:\\
\hline\\[-1em]
1.~~& \Write(x_1,0)\\
2.~~& \Write(x_1,0)\\
.~& \dots\\
2\cdot n-1.~~& \Write(x_n, 0)\\
2\cdot n.~~& \Write(x_n, 0)\\
\end{align*}
\end{subfigure}
\qquad
\begin{subfigure}[t]{0.15\textwidth}
\begin{align*}
\text{Thread}&~\Process_{2}:\\
\hline\\[-1em]
1.~~& \Read(x_1)\\
2.~~& \Read(x_2)\\
.~~& \dots\\
n.~~& \Read(x_n)
\end{align*}
\end{subfigure}
\caption{A toy program where $\VHB$ is exponentially coarser than $\Maz$.}
\label{fig:m_comparison2}
\end{figure}

==> figures/fig_comparison_viktor.tex <==
\begin{figure}[]
\small
\centering
\begin{subfigure}[b]{0.45\textwidth}
\centering
\begin{subfigure}[t]{0.15\textwidth}
\begin{align*}
\text{Th}&\text{read}~\Process_{1}:\\
\hline\\[-1em]
1.~& \Write(x,1)\\
2.~& \Write(x,1)\\
\,& \dots\\
n.~& \Write(x,1)
\end{align*}
\end{subfigure}
\qquad
\begin{subfigure}[t]{0.15\textwidth}
\begin{align*}
\text{Thread}&~\Process_{2}:\\
\hline\\[-1em]
1.~& \Write(x,2)\\
\,& \dots\\
n.~& \Write(x,2)\\
n+1.~& \Write(x,1)\\
n+2.~& \Read(x)\\
\,& \dots\\
2\cdot n+1.~~& \Read(x)
\end{align*}
\end{subfigure}
\caption{Many operations on one variable.}
\label{subfig:m_comparisona}
\end{subfigure}
\begin{subfigure}[b]{0.45\textwidth}
\centering
\begin{subfigure}[t]{0.15\textwidth}
\begin{align*}
\text{Thread}&~\Process_{1}:\\
\hline\\[-1em]
1.~~& \Write(x_1,1)\\
2.~~& \Write(x_1,1)\\
\,& \dots\\
2\cdot n-1.~~& \Write(x_n, n)\\
2\cdot n.~~& \Write(x_n, n)
\end{align*}
\end{subfigure}
\qquad
\begin{subfigure}[t]{0.15\textwidth}
\begin{align*}
\text{Thre}&\text{ad}~\Process_{2}:\\
\hline\\[-1em]
1.~~& \Read(x_1)\\
2.~~& \Read(x_2)\\
\,& \dots\\
n.~~& \Read(x_n)
\end{align*}
\end{subfigure}
\caption{Few operations on many variables.}
\label{subfig:m_comparisonb}
\end{subfigure}
\caption{Toy programs where $\VHB$ is exponentially coarser than $\Maz$.}
\label{fig:m_comparison}
\end{figure}
